Holding Secrets Accountable: Auditing Privacy-Preserving Machine Learning

Recent advancements in privacy-preserving machine learning are paving the way to extend the benefits of ML to highly sensitive data that, until now, have been hard to utilize due to privacy concerns and regulatory constraints. Simultaneously, there is a growing emphasis on enhancing the transparency and accountability of machine learning, including the ability to audit ML deployments. While ML auditing and PPML have both been the subjects of intensive research, they have predominately been examined in isolation. However, their combination is becoming increasingly important. In this work, we introduce Arc, an MPC framework for auditing privacy-preserving machine learning. At the core of our framework is a new protocol for efficiently verifying MPC inputs against succinct commitments at scale. We evaluate the performance of our framework when instantiated with our consistency protocol and compare it to hashing-based and homomorphic-commitment-based approaches, demonstrating that it is up to 10^4x faster and up to 10^6x more concise.

==> sections/extensions/pedersen_vector_commitments.tex <==


\subsection{Efficient Vector Comm. via EC-MPC}
\lsec{distcommit}


\begin{definition}[Pedersen Vector Commitments]
    \ldef{pvc}
    A Pedersen Vector Commitment for a vector of size $\sNumSamples$ in a cyclic group \sgroup of prime order $p$ with generators $\sgenerator_1,\ldots,\sgenerator_\sNumSamples$ and $h$
    consists of the following algorithms:
    \begin{algos}
        \item \(\textsf{PED.Setup}(1^\lambda, \sNumSamples) \rightarrow \pp\): Given a security parameter \( \lambda \), outputs \sgroup, its prime order $p$, and generators $\sgenerator_0,\ldots,\sgenerator_\sNumSamples$.

        \item \(\sPedCommit(\pp, (m_1, \ldots, m_\sNumSamples), r) \rightarrow \scommitment = r \cdot \sgenerator_0 + \sum_{i=1}^\sNumSamples m_i \cdot \sgenerator_i\).

        \item \(\sPedVerCommit(\pp, \scommitment, (m_1, \ldots, m_\sNumSamples), r) \rightarrow \{0, 1\}\): The verification checks that \( \scommitment \stackrel{?}{=} r \cdot \sgenerator_0 + \sum_{i=1}^\sNumSamples m_i \cdot \sgenerator_i \).

        \item $\sPedDistCommit(\pp, (\ssGeneric{\sInputs_1},\ldots,\ssGeneric{\sInputs_\sNumSamples}), \ssGeneric{r})$: Output $\scommitment$ by opening $\ssGeneric{\scommitment}$, where party $i$ computes $\ssGeneric{\scommitment}_i$ as:
    \begin{equation*}
        \ssGeneric{\scommitment}_i \leftarrow (\ssGeneric{r}_i \cdot h) \sum_{j=1}^\sNumSamples \ssGeneric{\sInputs_j}_i \cdot \sgenerator_{j-1}
    \end{equation*}
    \end{algos}
    Pedersen Vector Commitments are computationally binding and information-theoretically hiding~\cite{Bunz2018-mg}.
    For the binding property to hold, it is important that the \emph{trapdoors} $\strapdoor_1,\ldots,\strapdoor_\sNumSamples$ in $h = g_i^{\strapdoor_i}$ are unknown.
\end{definition}

A straightforward secure protocol to commit to a vector in a distributed fashion is to evaluate an arithmetic circuit emulating $\sPedCommit$ using an MPC protocol. 
To achieve better efficiency, we instead rely on an established technique, where the parties compute a circuit over the group $\mathbb{G}$ directly, thereby preventing overheads stemming from emulating group operations inside another algebraic structure~\cite{Smart2019-mpcec,Ozdemir2022-aw}. 

\begin{corollary}
    \lcol{distpedvec}
    Let \sprotocol be a secure protocol which computes a Pedersen Vector Commitment
    by evaluating an arithmetic circuit to emulate \sPedCommit.
    Let $\sprotocol^\prime$ be the same protocol, except that the commitment is computed
    using \sPedDistCommit. Then $\sprotocol^\prime$ is secure.
\end{corollary}
\begin{proof}
    We make use of Lemma 4 from~\cite{Ozdemir2022-aw}, which states that $\sprotocol^\prime$ is secure if the difference between
    $\sprotocol^\prime$ and $\sprotocol$ is a sub-circuit $C^\prime$ computing input wires to output wires according to a linear function $f$.
    In our case, we consider the function $C^\prime: \sfield_p^{\sNumSamples + 1} \leftarrow \sgroup$ that maps a decommitment value and a vector of inputs to a Pedersen Vector commitment,
    where the generators $\sgenerator_1,\ldots,\sgenerator_\sNumSamples$ and $h$ are public parameters. For ease of exposition, we set $\sgenerator_0 = h$.
    Observe that $C^\prime$ is linear, for two vectors of inputs $\sInputs^{(1)}, \sInputs^{(2)} \in \sfield_p^{\sNumSamples + 1}$ and two scalars $a, b \in \sfield_p$,
    $C^\prime(a \cdot \sInputs^{(1)} + b \cdot \sInputs^{(2)}) = \sum_{i=0}^\sNumSamples (a \cdot \sInputs^{(1)}_i + b \cdot \sInputs^{(2)}_i) \cdot \sgenerator_{j}=
    a \cdot \sum_{i=0}^\sNumSamples (\sInputs^{(1)}_i \cdot \sgenerator_{j}) + b \cdot \sum_{i=0}^\sNumSamples (\sInputs^{(2)}_i) \cdot \sgenerator_{j})
    = a \cdot C^\prime(\sInputs^{(1)}) + b \cdot C^\prime(\sInputs^{(2)})$.
    Hence, Lemma 4 implies that $\sprotocol^\prime$ is secure.

\end{proof}
